Kernel-based Tests for Joint Independence

We investigate the problem of testing whether $d$ random variables, which may or may not be continuous, are jointly (or mutually) independent. Our method builds on ideas of the two variable Hilbert-Schmidt independence criterion (HSIC) but allows for an arbitrary number of variables. We embed the $d$-dimensional joint distribution and the product of the marginals into a reproducing kernel Hilbert space and define the $d$-variable Hilbert-Schmidt independence criterion (dHSIC) as the squared distance between the embeddings. In the population case, the value of dHSIC is zero if and only if the $d$ variables are jointly independent, as long as the kernel is characteristic. Based on an empirical estimate of dHSIC, we define three different non-parametric hypothesis tests: a permutation test, a bootstrap test and a test based on a Gamma approximation. We prove that the permutation test achieves the significance level and that the bootstrap test achieves pointwise asymptotic significance level as well as pointwise asymptotic consistency (i.e., it is able to detect any type of fixed dependence in the large sample limit). The Gamma approximation does not come with these guarantees; however, it is computationally very fast and for small $d$, it performs well in practice. Finally, we apply the test to a problem in causal discovery.

==> Content/bootstrap.tex <==
\pagebreak
\section{Proof of permutation test consistency}


In this section we prove the consistency of the permutation test. Our
prove extends the results due to \citet{romano1989permutation} to
allow for function classes. To this end we use the following identity
\begin{equation*}
  \mhsic(\P)=\left(\sup_{f\in\prodRKHS:
      \norm{f}_{\prodRKHS}\leq 1}\abs[\big]{\Pjoint f-\Pprod f}\right)^2,
\end{equation*}
which follows by the characterization of $\mhsic$ via the maximum mean
discrepancy (MMD). Define the estimator
$T_n:\prodkernelspace^n\rightarrow\R$ for all $(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ by
\begin{equation*}
  T_n(\vx_1,\dots,\vx_n)\coloneqq \sqrt{n}\sup_{f\in\prodRKHS:
      \norm{f}_{\prodRKHS}\leq 1}\abs[\big]{\empjoint(\vx_1,\dots,\vx_n)f-\empprod(\vx_1,\dots,\vx_n)f},
\end{equation*}
then it is straightforward to see that $n\cdot\mhsicb_n=T_n^2$. Next
define for all $j\in\{1,\dots,d\}$ the sets
\begin{equation*}
  \mathcal{F}^j\coloneqq\{f\in\RKHS^j: \norm{f}_{\RKHS^j}\leq 1\}
\end{equation*}
and using the tensor product for vector spaces define the set
\begin{equation*}
\mathcal{F}\coloneqq\mathcal{F}^1\bar{\otimes}\cdots\bar{\otimes}\mathcal{F}^d\coloneqq\operatorname{span}\{f^1\otimes\cdots\otimes
f^d\,\mid\,\ f^1\in\mathcal{F}^1,\dots,f^d\in\mathcal{F}^d\}.
\end{equation*}
It can then be proved that
\begin{equation*}
  \overline{\mathcal{F}}=\{f\in\prodRKHS: \norm{f}_{\prodRKHS}\leq 1\}.
\end{equation*}
In particular, this implies that the estimator $T_n$ can be expressed
as
\begin{equation*}
  T_n(\vx_1,\dots,\vx_n)\coloneqq \sqrt{n}\sup_{f\in\mathcal{F}}\abs[\big]{\empjoint(\vx_1,\dots,\vx_n)f-\empprod(\vx_1,\dots,\vx_n)f}.
\end{equation*}
For $\P\in\pmspace{\kernelspace}$ and for
$\mathcal{G}\in\R^\kernelspace$ denote by $G_{\P}$ the centered Gaussian
process indexed by $\mathcal{G}$ with covariance function given for
all $f,g\in\mathcal{G}$ by
\begin{equation*}
  \operatorname{Cov}\left(G_{\P^j}f,G_{\P^j}g\right)=\E_{\P^j}(f(X)g(X))-\E_{\P^j}(f(X))\E_{\P^j}(g(X)).
\end{equation*}
Then, by \citet[Theorem 6]{sriperumbudur2013} it holds
that the function classes $\mathcal{F}^j$
satisfy the Donsker property, i.e. for all $\vX_1,\vX_2,\dots\iid\P$
it holds that
\begin{equation}
  \label{eq:Donsker1}
  \sqrt{n}\left(\empjoint^j(\vX_1,\dots,\vX_n)-\P^j\right)\overset{d}{\longrightarrow}G_{\P^j}
\end{equation}
as $n\rightarrow\infty$ in $\linfF$ where the convergence should be
taken with respect to the outer measure. Moreover, it also holds that
$\overline{\mathcal{F}}$, and hence $\mathcal{F}$, satisfies the Donsker
property, i.e. for all 
$\vX_1,\vX_2,\dots\iid\P$
it holds that
\begin{equation}
  \label{eq:Donsker2}
  \sqrt{n}\left(\empjoint(\vX_1,\dots,\vX_n)-\P\right)\overset{d}{\longrightarrow}G_{\P}
\end{equation}
as $n\rightarrow\infty$ in $\linfF$ where the convergence should be
taken with respect to the outer measure.
This also implies that $\mathcal{F}^j$ satisfies the
uniform Glivenko-Cantelli property, i.e.
\begin{equation*}
  \sup_{f\in\mathcal{F}^j}\abs[\big]{\empjoint^j(\vX_1,\dots,\vX_n)f-\P^jf}\overset{\P}{\longrightarrow}0,
\end{equation*}
as $n\rightarrow\infty$. A further proof of just the uniform
Glivenko-Cantelli property for compact state spaces $\kernelspace^j$
is given in \citet[Theorem 2.4]{mendelson2002}.

By use of the continuous mapping theorem it suffices to prove the
consistency of the permutation test for the test statistic $T_n$.
In order to prove this result we introduce the estimator
$S_n:\prodkernelspace^n\times\mathcal{F}\rightarrow\R$ defined for all
$(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ and for all $f\in\mathcal{F}$ by
\begin{equation*}
  S_n(\vx_1,\dots,\vx_n)f\coloneqq\sqrt{n}\left(\empjoint(\vx_1,\dots,\vx_n)f-\empprod(\vx_1,\dots,\vx_n)f\right).
\end{equation*}
Moreover, define the estimator $Z_n:\prodkernelspace^n\times\mathcal{F}\rightarrow\R$ for all
$(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ and for all $f=\sum_{i=1}^m\alpha_if_i^1\otimes\cdots\otimes
f_i^j\in\mathcal{F}$ by
\begin{equation*}
  Z_n(\vx_1,\dots,\vx_n)f\coloneqq\sqrt{n}\left(\empjoint(\vx_1,\dots,\vx_n)f-\sum_{j=1}^d\sum_{i=1}^m\alpha_i\bigg(\prod_{l\neq
      j}\P^l f_i^l\bigg)\empjoint^j(\vx_1,\dots,\vx_n)f_i^j+(d-1)\P f\right).
\end{equation*}
We begin by showing that $Z_n$ and $S_n$ have the same asymptotic
properties on $\linfF$.
\begin{lemma}[decomposition of $S_n$]
  \label{thm:decomposition_Sn}
  It holds for all $\P\in\HO$ and all
  $\vX_1,\vX_2,\dots\iid\P$ that
  \begin{equation*}
    \lim_{n\rightarrow\infty}\sup_{f\in\mathcal{F}}\abs{S_n(\vX_1,\dots,\vX_n)f-Z_n(\vX_1,\dots,\vX_n)f}=0.
  \end{equation*}
\end{lemma}

\begin{proof}
  Assume without loss of generality that for all $j\in\{1,\dots,d\}$
  it holds that $1\in\mathcal{F}^j$, else set
  $\mathcal{F}^{*j}\coloneqq\mathcal{F}^j\cup\{1\}$ and observe that
  the result for
  $\mathcal{F}^*\coloneqq\mathcal{F}^{*1}\bar{\otimes}\cdots\bar{\otimes}\mathcal{F}^{*d}$
  implies the result for $\mathcal{F}$.

  Fix $\P\in\HO$, $f\in\mathcal{F}$ and let $\vX_1,\vX_2,\dots\iid\P$. Then
  for all $j\in\{1,\dots,d\}$ it holds by the uniform
  Glivenko-Cantelli property of $\mathcal{F}^j$ that
  \begin{equation*}
    \sup_{f^j\in\mathcal{F}^j}\abs{\empjoint^j(\vX_1,\dots,\vX_n)f^j-\P^jf^j}\overset{\P}{\longrightarrow} 0,
  \end{equation*}
  as $n\rightarrow\infty$. Hence, using the continuity of the product
  together with the continuous mapping theorem it holds that
  \begin{equation*}
    \sup_{f\in\mathcal{F}}\abs{\empprod(\vX_1,\dots,\vX_n)f-\P f}\overset{\P}{\longrightarrow} 0,
  \end{equation*}
  as $n\rightarrow\infty$. Next, use the Hadamard differentiability
  \Niklas{add this result} to get that for all $f\in\mathcal{F}$ it
  holds that,
  \begin{equation*}
    S_n(\vX_1,\dots,\vX_n)f=Z_n(\vX_1,\dots,\vX_n)f+\landauo{1}.
  \end{equation*}
  This completes the proof of Lemma~\ref{thm:decomposition_Sn}.
\end{proof}

\begin{lemma}[asymptotic properties of $Z_n$]
  \label{thm:asymptotic_props_Zn}
  Let $\P_0\in\HO$ and $\vX_1,\vX_2\dots\iid\P_0$. Moreover, assume that
  $\boldsymbol{\pi}$ and $\boldsymbol{\pi}'$ are uniformly distributed
  on $(S_n)^d$ and
  $\boldsymbol{\pi}$, $\boldsymbol{\pi}'$ and $(\vX_i)_{i\in\N}$ are
  independent. Then it holds that
  \begin{equation*}
    \big(Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n)),Z_n(g_{n,\boldsymbol{\pi}'}(\vX_1,\dots,\vX_n))\big)
  \end{equation*}
  converges in distribution on $\linfF$ to a mean zero bivariate
  Gaussian process $(Z,Z')$ indexed by $\mathcal{F}$ such that $Z$ and $Z'$ have the same marginal
  distributions and for all $f\in\mathcal{F}$ it holds that $\operatorname{Cov}(Zf,Z'f)=0$.
\end{lemma}

\begin{proof}
  We begin by showing that
  $Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))$ converges to a mean
  zero Gaussian process $Z$. We can express $Z_n$ as
  a linear combination of empirical processes
  \begin{equation*}
    Z_n(\vX_1,\dots,\vX_n)=\sqrt{n}\left(\empjoint(\vX_1,\dots,\vX_n)-\P_0
      \right)-\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P_0^l\bigg)\sqrt{n}\left(\empjoint^j(\vX_1,\dots,\vX_n)-\P_0^j\right).
  \end{equation*}
  Therefore, we can apply \eqref{eq:Donsker1} and \eqref{eq:Donsker2} to
  get that
  \begin{equation*}
    Z_n(\vX_1,\dots,\vX_n)\overset{d}{\longrightarrow}G_{\P_0}-\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P_0^l\bigg)G_{\P_0^j}\eqqcolon Z,
  \end{equation*}
  as $n\rightarrow\infty$ in $\linfF$ (potentially
  using the outer measure due to measurability issues). Since $\P_0\in\HO$
  it holds that $Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))$ has
  the same distribution as $Z_n(\vX_1,\dots,\vX_n)$, therefore we have
  completed the first step.

  Next we analyze the asymptotic covariance. Fix
  $f=f^1\otimes\cdots\otimes f^d\in\mathcal{F}$ and
  $h=h^1\otimes\cdots\otimes h^d\in\mathcal{F}$ (by linearity of $Z_n$
  it will be sufficient to consider simple tensors). Moreover, define
  \begin{equation*}
    \psi(\vX_1,\dots,\vX_n)f\coloneqq\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P_0^lf^l\bigg)\empjoint^j(\vX_1,\dots,\vX_n)f^j.
  \end{equation*}
  Clearly, it holds that
  $\E\left(\empjoint(\vX_1,\dots,\vX_n)f\right)=\P_0 f$ and
  $\E\left(\psi(\vX_1,\dots,\vX_n)f\right)=d\cdot\P_0 f$. Hence, we get
  that
  \begin{align}
    &\operatorname{Cov}\left(Z_n(\vX_1,\dots,\vX_n)f,Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right)\nonumber\\
    &\quad=\operatorname{Cov}\bigg(\sqrt{n}\left(\empjoint(\vX_1,\dots,\vX_n)f-\psi(\vX_1,\dots,\vX_n)f\right),\nonumber\\
    &\qquad\qquad\qquad\sqrt{n}\left(\empjoint(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h-\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right)\bigg)\nonumber\\
    &\quad=n\E\bigg[\left(\empjoint(\vX_1,\dots,\vX_n)f-\psi(\vX_1,\dots,\vX_n)f\right)\nonumber\\
    &\qquad\qquad\qquad\left(\empjoint(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h-\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right)\bigg]-n(d-1)^2\cdot\P_0
    f\cdot\P_0 h.\label{eq:covariance_calculation}
  \end{align}
  In order to analyze the asymptotic properties of the expectation
  term we use the following identities:
  \begin{enumerate}[(i)]
  \item $\E\left[\empjoint(\vX_1,\dots,\vX_n)f\cdot\empjoint(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]=\P_0
    f\cdot\P_0 h+\landauo{n^{-1}}$\label{item:first_identity}
  \item $\E\left[\empjoint(\vX_1,\dots,\vX_n)f\cdot\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]=d\cdot\P_0
    f\cdot\P_0 h+\landauo{n^{-1}}$\label{item:proofitem}
  \item $\E\left[\psi(\vX_1,\dots,\vX_n)f\cdot\empjoint(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]=d\cdot\P_0
    f\cdot\P_0 h+\landauo{n^{-1}}$
  \item $\E\left[\psi(\vX_1,\dots,\vX_n)f\cdot\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]=d^2\P_0
    f\cdot\P_0 h+\landauo{n^{-1}}$\label{item:last_identity}
  \end{enumerate}
  The proofs for each are exactly the same. For illustration purposes
  we prove \eqref{item:proofitem}. Begin by using the independence
  assumption (i.e. $\P_0\in\HO$) we get
  \begin{align}
    &\E\left[\empjoint(\vX_1,\dots,\vX_n)f\cdot\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]\nonumber\\
    &\quad=\E\left[\left(\frac{1}{n}\sum_{i=1}^nf(\vX_i)\right)\left(\frac{1}{n}\sum_{i=1}^n\sum_{j=1}^d\bigg(\prod_{l\neq
          j}\P_0^lh^l\bigg)h^j(X_{\pi^j(i)}^j)\right)\right]\nonumber\\
    &\quad=\frac{1}{n^2}\sum_{i_1,i_2=1}^n\sum_{j=1}^d\E\left[\bigg(\prod_{l=1}^df^l(X_{i_1}^l)\bigg)\bigg(\prod_{l\neq
          j}\P_0^lh^l\bigg)h^j(X_{\pi^j(i_2)}^j)\right]\nonumber\\
    &\quad=\frac{1}{n^2}\sum_{i_1,i_2=1}^n\sum_{j=1}^d\bigg(\prod_{l\neq
          j}\P_0^lh^l\P_0^lf^l\bigg)\E\left[f^j(X_{i_1}^j)h^j(X_{\pi^j(i_2)}^j)\right]\label{eq:forwardequation}
  \end{align}
  Next, observe that we can express the expectation term by
  \begin{align*}
    &\E\left[f^j(X_{i_1}^j)h^j(X_{\pi^j(i_2)}^j)\right]\\
    &\quad=\E\left[f^j(X_{i_1}^j)\right]\E\left[h^j(X_{\pi^j(i_2)}^j)\right]\P\left[\pi^j(i_2)\neq
      i_1\right]+\E\left[f^j(X_{i_1}^j)h^j(X_{i_1}^j)\right]\P\left[\pi^j(i_2)=i_1\right]\\
    &\quad=\E\left[f^j(X_{i_1}^j)\right]\E\left[h^j(X_{\pi^j(i_2)}^j)\right]\frac{n-1}{n}+\E\left[f^j(X_{i_1}^j)h^j(X_{i_1}^j)\right]\frac{1}{n}\\
    &\quad=\E\left[f^j(X_{i_1}^j)\right]\E\left[h^j(X_{\pi^j(i_2)}^j)\right]+\landauo{n^{-1}},
  \end{align*}
  as $n\rightarrow\infty$. Hence, reversing the expansion in
  \eqref{eq:forwardequation} we get that
  \begin{align*}
    &\E\left[\empjoint(\vX_1,\dots,\vX_n)f\cdot\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]\\
    &\quad=\E\left[\empjoint(\vX_1,\dots,\vX_n)f\right]\E\left[\psi(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right]+\landauo{n^{-1}}\\
    &\quad=\P_0f\cdot P_0h+\landauo{n^{-1}}
  \end{align*}
  completing the proof of \eqref{item:proofitem}. We can now use the
  identities \eqref{item:first_identity}-\eqref{item:last_identity} in
  \eqref{eq:covariance_calculation} to get that
  \begin{align*}
    &\operatorname{Cov}\left(Z_n(\vX_1,\dots,\vX_n)f,Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))h\right)\\
    &\quad=n(1-d-d+d^2-(d-1)^2)\P_0f\cdot P_0h+\landauo{n^{-1}}\\
    &\quad=\landauo{n^{-1}}
  \end{align*}
  as $n\rightarrow\infty$.
  \Niklas{missing conclusion: we would need that if
    $X_n\overset{d}{\rightarrow}\mathcal{N}(0,1)$,
  $Y_n\overset{d}{\rightarrow}\mathcal{N}(0,1)$ and for all $n\in\N$,
$\operatorname{Cov}(X_n,Y_n)\rightarrow 0$ that it holds that
\begin{equation*}
  (X_n,Y_n)\overset{d}{\rightarrow}\mathcal{N}(0,Id_{2\times 2}).
\end{equation*}
Is this true?
}
\end{proof}

\begin{lemma}[asymptotic properties of $T_n$]
  \label{thm:asymptotic_props_Tn}
  Let $\P\in\pmspace{\prodkernelspace}$ and $\vX_1,\vX_2\dots\iid\P$. Moreover, assume that
  $\boldsymbol{\pi}$ and $\boldsymbol{\pi}'$ are uniformly distributed
  on $(S_n)^d$ and
  $\boldsymbol{\pi}$, $\boldsymbol{\pi}'$ and $(\vX_i)_{i\in\N}$ are
  independent. Then it holds that
  \begin{equation*}
    \big(T_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n)),T_n(g_{n,\boldsymbol{\pi}'}(\vX_1,\dots,\vX_n))\big)
  \end{equation*}
  converges in distribution to a random vector $(T,T')$ satisfying
  that $T$ and $T'$ are independent and identically
  distributed. Moreover, the distribution function $R(\cdot)$ of $T$
  is continuous and strictly increasing.
\end{lemma}

\begin{proof}
  Define the measure $\mathbb{Q}\coloneqq\Pprod\in\HO$ and observe that for
  $\tilde{\vX_1},\tilde{\vX}_2,\dots\iid\mathbb{Q}$ it holds that
  $g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n)$ has the same
  distribution under $\P$ as
  $g_{n,\boldsymbol{\pi}}(\tilde{\vX}_1,\dots,\tilde{\vX}_n)$ under
  $\mathbb{Q}$. Hence, we can apply
  Lemma~\ref{thm:asymptotic_props_Zn} to get that
    \begin{equation*}
    \big(Z_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n)),Z_n(g_{n,\boldsymbol{\pi}'}(\vX_1,\dots,\vX_n))\big)
  \end{equation*}
  converges in distribution on $\linfF$ to a mean zero bivariate
  Gaussian process $(Z,Z')$ indexed by $\mathcal{F}$ such that $Z$ and $Z'$ have the same marginal
  distributions and for all $f\in\mathcal{F}$ it holds that
  $\operatorname{Cov}(Zf,Z'f)=0$. Moreover, by
  Lemma~\ref{thm:decomposition_Sn} we can replace $Z_n$ by $S_n$.
  The continuous mapping theorem therefore implies that
  \begin{align*}
    &\big(T_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n)),T_n(g_{n,\boldsymbol{\pi}'}(\vX_1,\dots,\vX_n))\big)\\
    &\qquad=\big(\abs{S_n(g_{n,\boldsymbol{\pi}}(\vX_1,\dots,\vX_n))}_{\mathcal{F}},\abs{S_n(g_{n,\boldsymbol{\pi}'}(\vX_1,\dots,\vX_n))}_{\mathcal{F}}\big),
  \end{align*}
  converges in distribution to a random vector $(T,T')$ satisfying
  that $T$ and $T'$ are independent and identically
  distributed.
  \Niklas{Missing an argument showing that the distribution function
    of $T$ is strictly increasing. Worst case we can deal with this
    by considering the two possible $\xi_2$ cases.}  
\end{proof}


\begin{theorem}[consistency of the permutation test]
  \label{thm:consistencypermutationtest}
  Assume Setting \ref{setting:mHSIC} and let $\HO$ and $\HA$ be defined
  as in \eqref{eq:HO} and \eqref{eq:HA}, respectively. Then for all
  $\alpha\in(0,1)$ 
  the $\alpha$-permutation test is pointwise consistent when
  testing $\HO$ against $\HA$.
\end{theorem}

\begin{proof}
  Let $\P\in\HA$ and let
  $\hat{R}_{T_n}:\prodkernelspace^n\times\R\rightarrow [0,1]$ be the
  resampling distribution function corresponding to the test statistic
  $T$ and the resampling method
  $(g_{n,\boldsymbol{\pi}})_{\boldsymbol{\pi}\in(S_n)^d}$, i.e.
  \begin{equation*}
    \hat{R}_{T_n}(\vx_1,\dots,\vx_n)(t)\coloneqq\dfrac{1}{(n!)^d}\sum_{\boldsymbol{\pi}\in(S_n)^d}\mathds{1}_{\{T_n(g_{n,\boldsymbol{\pi}}(\vx_1,\dots,\vx_n))\leq
      t\}}.
  \end{equation*}
  By Lemma~\ref{thm:asymptotic_props_Tn} we satisfy
  all the requirements of \citet[Theorem 15.2.3]{lehmann} and hence get for $\vX_1,\vX_2,\dots\iid\P$ that
  \begin{equation*}
    \lim_{n\rightarrow\infty}\left(\hat{R}_{T_n}(\vX_1,\dots,\vX_n)\right)^{-1}(1-\alpha)=R^{-1}(1-\alpha),
  \end{equation*}
  where $R(\cdot)$ is the continuous and strictly increasing
  distribution function defined in
  Lemma~\ref{thm:asymptotic_props_Tn}. 
  In particular, this implies that
  there exists a $t^*\in\R$ such that
  \begin{equation}
    \label{eq:critvalbound}
    \sup_{n\in\N}\left(\hat{R}_{T_n}(\vX_1,\dots,\vX_n)\right)^{-1}(1-\alpha)\leq t^*.
  \end{equation}
  Moreover, by Theorem~\ref{thm:corollaryasymptoticdistmhsic} it holds
  for all $t\in\R$ that
  \begin{equation}
    \label{eq:asymptotic_divergence}
    \lim_{n\rightarrow\infty}\P\left(T_n(\vX_1,\dots,\vX_n)\leq t\right)=0.
  \end{equation}
  Using \eqref{eq:critvalbound} and \eqref{eq:asymptotic_divergence} the type II error can be bounded by
  \begin{align*}
    \limsup_{n\rightarrow\infty}\P(\phi_n(\vX_1,\dots,\vX_n)=0)&=\limsup_{n\rightarrow\infty}\P\left(T_n(\vX_1,\dots,\vX_n)\leq\left(\hat{R}_{T_n}(\vX_1,\dots,\vX_n)\right)^{-1}(1-\alpha)\right)\\
    &\leq\limsup_{n\rightarrow\infty}\P\left(T_n(\vX_1,\dots,\vX_n)\leq
      t^*\right)\\
    &=0,
  \end{align*}
  which completes the proof of Theorem~\ref{thm:consistencypermutationtest}.
\end{proof}

\pagebreak

\section{Proof of $\xi_2(h)>0$}

The proof uses the theory of empirical processes. We therefore
shortly recall some notation related to this theory, which mainly
builds on \citet{vandervaart}.

Let $\kernelspace$ be a measurable space, let
$\P\in\pmspace{\kernelspace}$ be a probability measure on this space
and let $\mathcal{G}$ be a function class consisting of measurable
functions $h:\kernelspace\rightarrow\R$. Moreover let
$X_1,X_2,\dots\iid\P$, which  due to issues related to the outer integral
defined below \citep[see also][Remark above Section
2.1.1]{vandervaart} are assumed to be canonically defined as
coordinate projections. The empirical measure
$\empjoint(X_1,\dots,X_n)\coloneqq\frac{1}{n}\sum_{i=1}^n\delta_{X_i}$
induces a linear map from $\mathcal{G}$ to $\R$ given by
\begin{equation*}
  h\mapsto\empjoint(X_1,\dots,X_n)h,
\end{equation*}
where we use the convention that
$\mathbb{Q}h\coloneqq\int_{\kernelspace} h(x) \measure{\mathbb{Q}}{x}$
for any measurable function $h$ and any signed measure $\mathbb{Q}$ on
$\kernelspace$.  A natural space to consider in this context is the
space of bounded functions from $\mathcal{G}$ to $\R$, which we denote
by $\linfG$. For all $T\in\linfG$ define the norm
$\norm{T}_{\mathcal{G}}\coloneqq\sup_{h\in\mathcal{G}}\abs{Th}$, then
the space $\linfG$ together with $\norm{\cdot}_{\mathcal{G}}$ forms a
Banach space which is separable if and only if $\mathcal{G}$
is a finite set. Assuming that for all $x\in\kernelspace$ it holds
that $\sup_{h\in\mathcal{G}}\abs{h(x)-\P h}<\infty$ allows us to view
the (normalized) empirical process
\begin{equation}
  \label{eq:empirical_process}
  \sqrt{n}\left(\empjoint(X_1,\dots,X_n)-\P\right),
\end{equation}
as an element of $\linfG$. In modern empirical process theory one
views this process as a random variable on $\linfG$ and is interested
in the asymptotic properties as $n\rightarrow\infty$. It, however,
turns out that the space $\linfG$ is in general too large to ensure
that the empirical process is a Borel measurable function. Therefore
it is common to introduce a specific outer integral, defined for all
functions $T$ from a probability space $(\Omega,\mathcal{F},\P)$ to
the extended real line $\overline{\R}$ (not necessarily measurable) by
\begin{equation*}
  \E^{*}(T)\coloneqq\inf\left\{\E(U):\, U\geq T,
    U:\Omega\rightarrow\overline{R}\text{ measurable and }\E(U)\text{ exists}\right\}.
\end{equation*}
Based on this definition one can extend the notions of convergence in
distribution, probability and almost surely \citep[Chapter
1]{vandervaart}. For example, assume $(X_n)_{n\in\N}$ is a sequence of
possibly non-measurable functions from underlying probability spaces
$(\Omega_n,\mathcal{A}_n,\P_n)$ to a metric space $\kernelspace$ and
let $X$ be a Borel measurable map on $\kernelspace$. Then we say
$(X_n)_{n\in\N}$ converges weakly in $\kernelspace$ to $X$, and write
$X_n\rightsquigarrow_{\kernelspace} X$, if for all
$f\in\operatorname{C}_b(\kernelspace)$ it holds that
\begin{equation*}
  \lim_{n\rightarrow\infty}\E^{*}(f(X_n))=\E(f(X)).
\end{equation*}

An important aspect of empirical process theory is to classify the
sets $\mathcal{G}$ in which the
empirical process defined in \eqref{eq:empirical_process} converges
weakly in $\linfG$. To this end, we need to introduce a particular
Gaussian process. For a probability distribution
$\P\in\pmspace{\kernelspace}$ and for a class of functions
$\mathcal{G}\subset\Lpspace{2}{\P}{\abs{\cdot}_{\R}}$ denote by
$G_{\P}$ the centered Gaussian process indexed by $\mathcal{G}$ with
covariance function given for all $f,g\in\mathcal{G}$ by
\begin{equation*}
  \operatorname{Cov}\left(G_{\P}f,G_{\P}g\right)=\E_{\P}(f(X)g(X))-\E_{\P}(f(X))\E_{\P}(g(X)).
\end{equation*}
The process $G_{\P}$ is sometimes called (generalized)
Brownian bridge process.

It should be clear that convergence of the empirical process is
related to the size of the function class $\mathcal{G}$. We call a
class of functions $\mathcal{G}$ a $\P$-Donsker class if for
$X_1,X_2,\dots\iid\P$ it holds that
\begin{equation*}
  \sqrt{n}\left(\empjoint(X_1,\dots,X_n)-\P\right)\rightsquigarrow_{\linfG} G_{\P}
\end{equation*}
as $n\rightarrow\infty$ and $G_{\P}$ is a tight Borel measurable
element in $\linfG$.

We now turn back to dHSIC. Denote by
$\empprod(\vx_1,\dots,\vx_n)\coloneqq\prod_{j=1}^d\left(\frac{1}{n}\sum_{i=1}^n\delta_{x^j_i}\right)$
the empirical product distribution and define the estimator $T_n:\prodkernelspace^n\rightarrow\R$ for all
$(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ by
\begin{equation*}
  T_n(\vx_1,\dots,\vx_n)\coloneqq \sqrt{n}\sup_{f\in\prodRKHS:
    \norm{f}_{\prodRKHS}\leq 1}\abs[\big]{\empjoint(\vx_1,\dots,\vx_n)f-\empprod(\vx_1,\dots,\vx_n)f},
\end{equation*}
then it is straightforward to prove that
$n\cdot\mhsicb_n=(T_n)^2$. Next, define for all $j\in\{1,\dots,d\}$ the
sets $\mathcal{F}^j\coloneqq\{f\in\RKHS^j: \norm{f}_{\RKHS^j}\leq 1\}$
and using the tensor product for functions define the set
\begin{equation}
  \label{eq:general_functionclass_F}
  \mathcal{F}\coloneqq\left\{f=\sum_{l=1}^m\lambda_lf^1_l\otimes\cdots\otimes
  f^d_l\,\Big\rvert\,\sum_{l=1}^m\lambda_l\leq 1\text{, }\lambda_l\geq 0\text{
    and } f^j_l\in\mathcal{F}^j\right\}.
\end{equation}
By \citet[Proposition 2.2]{ryan} it holds that $\overline{\mathcal{F}}=\{f\in\prodRKHS:
\norm{f}_{\prodRKHS}\leq 1\}$, which in particular, implies that the
estimator $T_n$ can be expressed as
\begin{equation*}
  T_n(\vx_1,\dots,\vx_n)\coloneqq \sqrt{n}\sup_{f\in\mathcal{F}}\abs[\big]{\empjoint(\vx_1,\dots,\vx_n)f-\empprod(\vx_1,\dots,\vx_n)f}.
\end{equation*}
Introduce the estimator
$S_n:\prodkernelspace^n\rightarrow\linfF$ defined for all
$(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ by
\begin{equation*}
  S_n(\vx_1,\dots,\vx_n)\coloneqq\sqrt{n}\left(\empjoint(\vx_1,\dots,\vx_n)-\empprod(\vx_1,\dots,\vx_n)\right).
\end{equation*}
The idea is to use the empirical process theory to find a weak limit
for $S_n$. By the continuous mapping theorem this will give us a weak
limit of $T_n=\norm{S_n}_{\mathcal{F}}$. In order to apply the empirical process theory, we show
that $S_n$ can be approximated by the estimator
$Z_n:\prodkernelspace^n\rightarrow\linfF$ which is defined for all
$(\vx_1,\dots,\vx_n)\in\prodkernelspace^n$ by
\begin{equation*}
  Z_n(\vx_1,\dots,\vx_n)\coloneqq\sqrt{n}\left(\empjoint(\vx_1,\dots,\vx_n)-\prodlawbold
  \right)-\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P^{X^l}\bigg)\sqrt{n}\left(\empjoint^j(\vx_1,\dots,\vx_n)-\P^{X^j}\right).
\end{equation*}
This trick, of approximating $S_n$ by a linear combination of
normalized empirical processes, is due to
\citet{romano1988bootstrap}. We will then be able to show that $Z_n$ converges to
a Gaussian process by making use of \citet[Theorem
6]{sriperumbudur2013}, which states that for all $j\in\{1,\dots,d\}$
the function class $\mathcal{F}^j$ is a $\P^{X^j}$-Donsker
class and also that the function class $\overline{\mathcal{F}}$, and
hence also $\mathcal{F}$, is a $\prodlawbold$-Donsker class.

We begin by showing that $Z_n$ and $S_n$ have the same asymptotic
properties on $\linfF$. The proof of this Lemma extends the ideas in
\citet{romano1988bootstrap} to account for classes of functions
instead of sets. Moreover, for the convergence we make use
of the empirical process theory.
\begin{lemma}[decomposition of $S_n$]
  \label{thm:decomposition_Sn}
  Assume Setting~\ref{setting:mHSIC}. Then for all
  $\vX_1,\vX_2,\dots\iid\prodlawbold\in\HO$ it holds that 
  \begin{equation*}
    \norm{S_n(\vX_1,\dots,\vX_n)-Z_n(\vX_1,\dots,\vX_n)}_{\mathcal{F}}\overset{\P}{\longrightarrow}0,
  \end{equation*}
  as $n\rightarrow\infty$.
\end{lemma}

\begin{proof}
  % Assume without loss of generality that for all $j\in\{1,\dots,d\}$
  % it holds that $1\in\mathcal{F}^j$, else set
  % $\mathcal{F}^{*j}\coloneqq\mathcal{F}^j\cup\{1\}$ and observe that
  % the result for
  % $\mathcal{F}^*$, defined as in \eqref{eq:general_functionclass_F}
  % with $\mathcal{F}^j$ replaced by $\mathcal{F}^{*j}$ for all $j\in\{1,\dots,d\}$,
  % implies the result for $\mathcal{F}$. Moreover, by the linearity of
  % the maps given in \eqref{eq:measure_map}, it is sufficient to
  % consider functions of the form $f=f^1\otimes\dots\otimes f^d\in\mathcal{F}$.
  Fix $\vX_1,\vX_2,\dots\iid\prodlawbold\in\HO$ and denote by
  $\empjoint^j(\vx_1,\dots,\vx_n)\coloneqq\frac{1}{n}\sum_{i=1}^n\delta_{x^j_i}$
  the empirical measure on the $j$-th coordinate. Then for all $j\in\{1,\dots,d\}$ it holds by
  \citet[Theorem 6]{sriperumbudur2013} that $\mathcal{F}^j$ is a
  $\P^{X^j}$-Donsker class and hence in particular that
  \begin{equation*}
    \norm[\big]{\empjoint^j-\P^{X^j}}_{\mathcal{F}^j}\coloneqq\sup_{h\in\mathcal{F}^j}\abs[\big]{\empjoint^j(\vX_1,\dots,\vX_n)h-\P^{X^j}h}=\landauProbO{n^{-\frac{1}{2}}},
  \end{equation*}
  as $n\rightarrow\infty$.
  % Hence, using the continuity of the product
  % together with the continuous mapping theorem it holds that
  % \begin{align}
  %   \norm{\empprod(\vX_1,\dots,\vX_n)-\prodlawbold}_{\mathcal{F}}=&\sup_{h\in\mathcal{F}}\abs{\empprod(\vX_1,\dots,\vX_n)h-\prodlawbold
  %     h}\nonumber\\
  %   &=\sup_{h\in\mathcal{F}}\abs[\bigg]{\sum_{l=1}^m\lambda_l\bigg(\prod_{j=1}^d\empjoint^j(\vX_1,\dots,\vX_n)h^j_l-\prod_{j=1}^d\P^{X^j}h^j_l\bigg)}\nonumber\\
  %   &\leq
  %   \sup_{h\in\mathcal{F}}\abs[\bigg]{\sum_{l=1}^m\bigg[\prod_{j=1}^d\bigg(\empjoint^j(\vX_1,\dots,\vX_n)h^j_l-\P^{X^j}h^j_l+\P^{X^j}h^j_l\bigg)-\prod_{j=1}^d\P^{X^j}h^j_l\bigg]}\nonumber\\
  %   &\leq\sum_{l=1}^m\abs[\bigg]{}\label{eq:glivenko_type_prop}
  % \end{align}
  % as $n\rightarrow\infty$.
  Next, let
  $f=f^1\otimes\dots\otimes
  f^d\in\mathcal{F}$ then it holds that
  \begin{align}
    \empprod(\vX_1,\dots,\vX_n)f&=\prod_{j=1}^d\empjoint^j(\vX_1,\dots,\vX_n)f^j\nonumber\\
    &=\prod_{j=1}^d\left[\P^{X^j}f^j+\left(\empjoint^j(\vX_1,\dots,\vX_n)f^j-\P^{X^j}f^j\right)\right]\nonumber\\
    &=\prodlawbold
      f+\sum_{j=1}^d\left(\prod_{k\neq
          j}\P^{X^k}f^k\right)\left(\empjoint^j(\vX_1,\dots,\vX_n)f^j-\P^{X^j}f^j\right)+R\left(\empprod,\prodlawbold,f\right),\label{eq:decompositionSn_1}
  \end{align}
  where $R\left(\empprod,\prodlawbold,f\right)$ is the remainder
  term resulting from multiplying out the product. In order to
  quantify the contribution of this remainder term to the sum,
  observe that for all $j\in\{1,\dots,d\}$ it holds that
  \begin{equation}
    \label{eq:remainderterm_est_1}
    \abs[\big]{\empjoint^j(\vX_1,\dots,\vX_n)f^j-\P^{X^j}f^j}
    \leq\norm[\big]{\empjoint^j(\vX_1,\dots,\vX_n)-\P^{X^j}}_{\mathcal{F}^j}
    =\landauProbO{n^{-\frac{1}{2}}}
  \end{equation}
  as $n\rightarrow\infty$. Moreover, using that $\mathcal{F}^j$
  consists of uniformly bounded functions (clearly true since
  $\mathcal{F}^j$ is the unit ball of the RKHS $\RKHS^j$) it holds that
  \begin{equation}
    \label{eq:remainderterm_est_2}
    \abs[\big]{\P^{X^j}f^j}
    \leq\norm[\big]{\P^{X^j}}_{\mathcal{F}^j}<\infty.
  \end{equation}
  Now, since $R\left(\empprod,\prodlawbold,f\right)$ only contains
  terms with at least two factors of the form
  $\left(\empjoint^kf^k_l-\P^{X^k}f^k_l\right)$ it holds by
  \eqref{eq:remainderterm_est_1} and \eqref{eq:remainderterm_est_2} that
  \begin{equation}
    \label{eq:decompositionSn_2}
    \abs[\Big]{R\left(\empprod,\prodlawbold,f\right)}=\landauProbO{n^{-1}}.
  \end{equation}
  as $n\rightarrow\infty$. Finally, using \eqref{eq:decompositionSn_1} and
  \eqref{eq:decompositionSn_2} we get for all
  $f=\sum_{l=1}^m\lambda_lf^1_l\otimes\dots\otimes
  f^d_l\in\mathcal{F}$ that
  \begin{align*}
    &\abs{S_n(\vX_1,\dots,\vX_n)f-Z_n(\vX_1,\dots,\vX_n)f}\\
    &\quad=\abs[\bigg]{\sum_{l=1}^m\lambda_l\sqrt{n}\Big[\prodlawbold
        f_l-\empprod(\vX_1,\dots,\vX_n) f_l+\sum_{j=1}^d\Big(\prod_{k\neq
          j}\P^{X^k}f^k_l\Big)\Big(\empjoint^j(\vX_1,\dots,\vX_n)f^j_l-\P^{X^j}f^j_l\Big)\Big]}\\
    &\quad=\abs[\bigg]{\sum_{l=1}^m\lambda_l\sqrt{n}R\left(\empprod,\prodlawbold,f_l\right)}\\
    &\quad=\landauProbO{n^{-\frac{1}{2}}},
  \end{align*}
  as $n\rightarrow\infty$. Since the bound is independent of $f$ we
  immediately get
  \begin{equation*}
    \norm{S_n(\vX_1,\dots,\vX_n)-Z_n(\vX_1,\dots,\vX_n)}_{\mathcal{F}}\overset{\P}{\longrightarrow}0,
  \end{equation*}
  as $n\rightarrow\infty$, which completes the proof of Lemma~\ref{thm:decomposition_Sn}.
  % \begin{align}
  %   \abs[\big]{\empjoint^j(\vX_1,\dots,\vX_n)f^j-\P^{X^j}f^j}
  %   &=\abs[\bigg]{\int_{\prodkernelspace}f^j(x^j)\measure{\left(\empprod(\vX_1,\dots,\vX_n)-\prodlawbold\right)}{\vx}}\nonumber\\
  %   &\leq\sup_{h\in\mathcal{F}}\abs[\bigg]{\int_{\prodkernelspace}h(\vx)\measure{\left(\empprod(\vX_1,\dots,\vX_n)-\prodlawbold\right)}{\vx}}\nonumber\\
  %   &=\norm[\big]{\empprod(\vX_1,\dots,\vX_n)-\prodlawbold}_{\mathcal{F}},\label{eq:remainderterm_est_1}
  % \end{align}
  % where we used the assumption that $1\in\mathcal{F}^j$ for all
  % $j\in\{1,\dots,d\}$. Moreover, by a similar argument and using that
  % $\mathcal{F}$ consists of uniformly bounded functions (clearly true
  % for the unit ball in $\prodRKHS$) it holds that
  % \begin{equation}
  %   \label{eq:remainderterm_est_2}
  %   \abs[\big]{\P^{X^j}f^j}
  %   =\abs[\bigg]{\int_{\prodkernelspace}f^j(x^j)\measure{\prodlawbold}{\vx}}
  %   \leq\sup_{h\in\mathcal{F}}\abs[\bigg]{\int_{\prodkernelspace}h(\vx)\measure{\prodlawbold}{\vx}}
  %   =\norm[\big]{\prodlawbold}_{\mathcal{F}}<\infty.
  % \end{equation}
  % Now, since $R\left(\empprod,\prodlawbold,f\right)$ only contains
  % terms with at least two factors of the form
  % $\left(\empjoint^kf^k_l-\P^{X^k}f^k_l\right)$ it holds by
  % \eqref{eq:remainderterm_est_1} and \eqref{eq:remainderterm_est_2} that
  % there exist constants $0\leq C_2,\dots,C_d<\infty$ such that
  % \begin{equation}
  %   \label{eq:decompositionSn_2}
  %   \abs[\Big]{R\left(\empprod,\prodlawbold,f\right)}\leq \sum_{j=2}^d\norm{\empprod(\vX_1,\dots,\vX_n)-\prodlawbold}_{\mathcal{F}}^jC_j.
  % \end{equation}
  % By \eqref{eq:glivenko_type_prop} this implies that there exists a
  % $0\leq C<\infty$ such that $R\left(\empprod,\prodlawbold,f\right)$
  % is asymptotically bounded by
  % $C\norm{\empprod(\vX_1,\dots,\vX_n)-\prodlawbold}_{\mathcal{F}}^2$.

  % Using \eqref{eq:decompositionSn_1} and
  % \eqref{eq:decompositionSn_2} we get for all
  % $f=\sum_{l=1}^m\lambda_lf^1_l\otimes\dots\otimes
  % f^d_l\in\mathcal{F}$ that
  % \begin{align*}
  %   \abs{S_nf-Z_nf}
  %   &=\abs[\bigg]{\sum_{l=1}^m\lambda_l\sqrt{n}\Big[\prodlawbold
  %       f_l-\empprod f_l+\sum_{j=1}^d\Big(\prod_{k\neq
  %         j}\P^{X^k}f^k_l\Big)\Big(\empjoint^jf^j_l-\P^{X^j}f^j_l\Big)\Big]}\\
  %   &=\abs[\bigg]{\sum_{l=1}^m\lambda_l\sqrt{n}R\left(\empprod,\prodlawbold,f_l\right)}
  % \end{align*}
\end{proof}

\begin{lemma}[asymptotic properties of $Z_n$]
  \label{thm:asymptotic_props_Zn2}
  Assume Setting~\ref{setting:mHSIC}. Let
  $\vX_1,\vX_2\dots\iid\prodlawbold\in\HO$. Then it holds that
  \begin{equation*}
    Z_n(\vX_1,\dots,\vX_n)
  \end{equation*}
  converges in distribution on $\linfF$ to a centered Gaussian
  process $Z$ indexed by $\mathcal{F}$ such that $Z$ is a tight Borel
  measurable element on $\linfF$ and such that $\P\left(\norm{Z}_{\mathcal{F}}=0\right)=0$.
\end{lemma}

\begin{proof}
  Recall that $Z_n$ (first introduced by \citet{romano1988bootstrap}) is a linear combination of empirical processes
  \begin{equation}
    \label{eq:Zn_rep_emp_process}
    Z_n(\vX_1,\dots,\vX_n)=\sqrt{n}\left(\empjoint(\vX_1,\dots,\vX_n)-\prodlawbold
      \right)-\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P^{X^l}\bigg)\sqrt{n}\left(\empjoint^j(\vX_1,\dots,\vX_n)-\P^{X^j}\right).
  \end{equation}
  Therefore, since by \citet[Theorem 6]{sriperumbudur2013} for all
  $j\in\{1,\dots,d\}$ the sets $\mathcal{F}^j$ are $\P^{X^j}$-Donsker
  classes and $\mathcal{F}$ is a $\prodlawbold$-Donsker class it holds
  that
  \begin{equation*}
    Z_n(\vX_1,\dots,\vX_n)\rightsquigarrow_{\linfF} G_{\prodlawbold}-\sum_{j=1}^d\bigg(\prod_{l\neq
    j}\P^{X^l}\bigg)G_{\P^{X^j}}\eqqcolon Z,
  \end{equation*}
  as $n\rightarrow\infty$. Using that the sum of tight
  Borel measurable Gaussian processes is again a tight Borel
  measurable Gaussian process, it follows that $Z$ is a tight Borel
  measurable centered Gaussian process on $\linfF$.
  
  It remains to show that $\P\left(\norm{Z}_{\mathcal{F}}=0\right)=0$. By
  monotonicity of the integral it is enough to show that there exists
  $f_0\in\mathcal{F}$ such that $\P\left(\abs{Zf_0}=0\right)=0$.  To
  this end, define for all $f=f^1\otimes\dots\otimes
  f^d\in\mathcal{F}$ and for all $i\in\N$ the random variables
  \begin{equation*}
    Y_i(f)\coloneqq
    f(\vX_i)-\E\left(f(\vX_i)\right)-\sum_{j=1}^d\left(\prod_{l\neq j}\E\left(f^l(X^l_i)\right)\right)\left(f^j(X^j_i)-\E\left(f^j(X^j_i\right)\right).
  \end{equation*}
  Clearly, it holds that $(Y_i(f))_{i\in\N}$ is an iid sequence of
  centered real-valued random variables and by
  \eqref{eq:Zn_rep_emp_process} it holds that
  $Z_nf=\frac{1}{\sqrt{n}}\sum_{i=1}^nY_i(f)$.
  Hence, if we are able to show that there exists
  $f_0=f^1_0\otimes\dots\otimes f^d_0\in\mathcal{F}$
  such that $\Var\left(Y_i(f_0)\right)>0$ the classical central limit
  theorem proves that $\P\left(\abs{Zf_0}=0\right)=0$. Using that
  $\prodlawbold\in\HO$ we can perform the following calculation.
  \begin{align}
    \Var\left(Y_i(f)\right)
    &=\E\Bigg(\Big[f(\vX_i)-\sum_{j=1}^d\Big(\prod_{l\neq
            j}\E\left(f^l(X^l_i)\right)\Big)f^j(X^j_i)\Big]^2\Bigg)-(d-1)^2\E\left(f(\vX_i)\right)^2\nonumber\\
    &=\E\left(f(\vX_i)^2\right)-\sum_{j=1}^d\Big(\prod_{l\neq
            j}\E\left(f^l(X^l_i)\right)\Big)\E\left(f(\vX_i)f^j(X^j_i)\right)\nonumber\\
    &\quad +\sum_{j_1=1}^d\sum_{j_2=1}^d\Big(\prod_{l_1\neq
      j_1}\E\left(f^{l_1}(X^{l_1}_i)\right)\Big)\Big(\prod_{l_2\neq
      j_2}\E\left(f^{l_2}(X^{l_2}_i)\right)\Big)\E\left(f^{j_1}(X^{j_1}_i)f^{j_2}(X^{j_2}_i)\right)\nonumber\\
    &\quad -(d-1)^2\E\left(f(\vX_i)\right)^2\nonumber\\
    &=\E\left(f(\vX_i)^2\right)-\sum_{j=1}^d\Big(\prod_{l\neq
            j}\E\left(f^l(X^l_i)\right)\Big)^2\E\left(f^j(X^j_i)^2\right)\nonumber\\
    &\quad +\sum_{j=1}^d\Big(\prod_{l\neq
            j}\E\left(f^l(X^l_i)\right)\Big)^2\E\left(f^j(X^j_i)^2\right)+d(d-1)\E\left(f(\vX_i)\right)^2-(d-1)^2\E\left(f(\vX_i)\right)^2\nonumber\\
    &=\Var\left(f(\vX_i)\right)+d\cdot\E\left(f(\vX_i)\right)^2.\label{eq:variance_yi}
  \end{align}
  Assume for the sake of contradiction that
  $\E\left(f(\vX_i)\right)=0$ for all $f=f^1\otimes\dots\otimes
  f^d\in\mathcal{F}$, then by linearity it in particular holds that
  $\E\left(f(\vX_i)\right)=0$ for all $f\in\mathcal{F}$. Using the
  properties of the Bochner integral and the definition of the mean
  embedding function this implies that for all $f\in\mathcal{F}$ it
  holds that
  \begin{equation*}
    \E\left(f(\vX_i)\right)
    =\E\Big(\scalarprod[\big]{\prodk(\vX_i,\cdot),f}_{\prodRKHS}\Big)
    =\scalarprod[\big]{\Pi\left(\prodlawbold\right),f}_{\prodRKHS}=0.
  \end{equation*}
  Since $\overline{\mathcal{F}}$ is the unit ball in $\prodRKHS$ it
  holds that $\Pi\left(\prodlawbold\right)=0$. By
  Setting~\ref{setting:mHSIC}, we have that $\Pi$ is injective (since
  $\prodk$ is characteristic) and hence $\prodlawbold\equiv 0$, which
  contradicts that $\prodlawbold$ is a probability
  distribution. Therefore, there exists $f_0=f^1_0\otimes\dots\otimes
  f^d_0\in\mathcal{F}$ such that $\E\left(f_0(\vX_i)\right)^2>0$. By
  \eqref{eq:variance_yi} this implies that
  $\Var\left(f_0(\vX_i)\right)>0$, which completes the proof of
  Lemma~\ref{thm:asymptotic_props_Zn2}.
\end{proof}

\begin{theorem}[continuous asymptotic distribution]
  \label{thm:cont_strictly_increasing_cdf}
  Assume Setting~\ref{setting:mHSIC}. Then for
  $\vX_1,\vX_2,\dots\iid\prodlawbold\in\HO$ it holds that
  \begin{equation*}
    n\cdot\mhsicb\left(\vX_1,\dots,\vX_n\right)
  \end{equation*}
  converges in distribution to a random variable with distribution
  function continuous on $(0,\infty)$.
\end{theorem}

\begin{proof}
  It is sufficient to prove the result for $T_n$, because
  $n\cdot\mhsicb_n=(T_n)^2$. Furthermore, by
  Lemma~\ref{thm:decomposition_Sn} and
  Lemma~\ref{thm:asymptotic_props_Zn2} it holds that
  $S_n(\vX_1,\dots,\vX_n)$ converges in distribution on $\linfF$ to a
  mean zero Gaussian process $Z$ indexed by $\mathcal{F}$ such that
  $Z$ is a tight Borel measurable element in $\linfF$.  Next, by
  \citet[Lemma 1.5.9]{vandervaart2} there exists a semi-metric $\rho$
  on $\mathcal{F}$ for which the paths of $Z$ are $\P$-a.s. uniformly
  continuous and $\mathcal{F}$ is totally bounded.

  Denote by $\operatorname{C}_u(\mathcal{F},\rho)$ the space of
  bounded uniformly continuous functions from $\mathcal{F}$ to
  $\R$. It can be shown that this space seen as a subspace of $\linfF$
  with the $\norm{\cdot}_{\mathcal{F}}$ norm is a complete and separable
  space if $\mathcal{F}$ is totally bounded with respect to $\rho$
  \citep[e.g.][Example 18.7]{vandervaart}. The previous considerations
  therefore imply that it holds $\P$-a.s. that $Z$ takes values in a
  separable Banach space.  Therefore we can apply \citet[Exercise
  2.4.4]{gine} with $B=\operatorname{C}_u(\mathcal{F},\rho)$, which proves that
  distribution function of $\norm{Z}_{\mathcal{F}}$ is continuous on
  $(0,\infty)$.  Moreover, the continuous mapping theorem \citep[for an
  extention to outer measures see][Theorem 1.11.1]{vandervaart2}
  together with the continuity of the norm implies that $T_n$
  converges in distribution to $\norm{Z}_{\mathcal{F}}$. This completes the
  proof of Theorem~\ref{thm:cont_strictly_increasing_cdf}.
  % \Niklas{show that $Z$ is non-degenerate -->
  %   IMPORTANT} Applying a structure theorem for Gaussian measures
  % \citep[e.g.][Theorem 8.2.5]{stroock}, we get an abstract Wiener space. We
  % are therefore in the setting of \citet[Proposition 2]{beran1986}, which
  % proves that $\abs{Z}_{\infty}$ has a continuous distribution with
  % strictly increasing distribution function. Using the continuous
  % mapping theorem \citep[for an extention to outer measures
  % see][Theorem 1.11.1]{vandervaart2} together with the continuity of the norm implies
  % that $T_n$ converges in distribution to $\abs{Z}_{\infty}$. This
  % completes the proof of Theorem~\ref{thm:cont_strictly_increasing_cdf}.
\end{proof}

\begin{corollary}[$\xi_2(h)>0$]
  \label{thm:xi2greater2}
  Assume Setting~\ref{setting:mHSIC} and recall \eqref{eq:xi_c}. Then it holds that
  \begin{equation*}
    \xi_2(h)>0.
  \end{equation*}
\end{corollary}

\begin{proof}
  Assume $\xi_2(h)=0$. Then, by Theorem~\ref{thm:asymptoticdist_HO} it
  holds that $n\cdot\mhsicb_n$ converges to constant. Slutsky's
  theorem together with Lemma~\ref{thm:decomposition_Sn} and
  Lemma~\ref{thm:asymptotic_props_Zn2} proves that this constant
  cannot be $0$. This however contradicts
  Theorem~\ref{thm:cont_strictly_increasing_cdf}, which states that
  the limiting distribution of $n\cdot\mhsicb_n$ has a distribution
  function which is continuous on $(0,\infty)$. Hence $\xi_2(h)>0$,
  which completes the proof of Corollary~\ref{thm:xi2greater2}.
\end{proof}


\pagebreak


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../dHSIC_main"
%%% End: 

